Know Your Space: Inlier and Outlier Construction for Calibrating Medical OOD Detectors

We focus on the problem of producing well-calibrated out-of-distribution (OOD) detectors, in order to enable safe deployment of medical image classifiers. Motivated by the difficulty of curating suitable calibration datasets, synthetic augmentations have become highly prevalent for inlier/outlier specification. While there have been rapid advances in data augmentation techniques, this paper makes a striking finding that the space in which the inliers and outliers are synthesized, in addition to the type of augmentation, plays a critical role in calibrating OOD detectors. Using the popular energy-based OOD detection framework, we find that the optimal protocol is to synthesize latent-space inliers along with diverse pixel-space outliers. Based on empirical studies with multiple medical imaging benchmarks, we demonstrate that our approach consistently leads to superior OOD detection ($15\% - 35\%$ in AUROC) over the state-of-the-art in a variety of open-set recognition settings.

==> conclusion.tex <==







% Ensuring safety and reliability of AI based models in applications such as healthcare is of paramount importance. While model safety encompasses a broad range of objectives (e.g., calibration, adversarial robustness, resilience to data biases etc.), in this paper, we focused on anomaly detection methods that can help avoid models from being blindsided when deployed in the open-world and guide practitioners in decision making. We test our approach using a variety of real-world medical imaging benchmarks. However, we acknowledge that our method may be insufficient when dealing with other types of real-world domain shifts or uncontrollable factors that affect the characteristics of data. We believe our work adds to the growing efforts in the field of anomaly detection and can also motivate further research in the healthcare community at large. 

  



% model safety is critical important problem. instead of model misusue, avoid models from being blind sides. thats our main focus. it will be imapctful. of course there are real world shifts, our method may be insufficient. uncontrollable variations and factors, but definitely research in the healthcare community

==> results.tex <==


\paragraph{Far OOD Detection on MedMNIST.} All methods were trained with a $40-2$ WideResNet feature extractor backbone~\cite{zagoruyko2016wide}. In each experiment, one of the $8$ datasets was considered as ID and the OOD detection performance was evaluated using the remaining datasets. In Table \ref{tab:s+d_medmnist}, we report the mean and standard deviations of AUROC scores for the different approaches. It can be observed that our approach consistently outperforms all baselines by significant margins. Interestingly, state-of-the-art baselines such as G-ODIN and VOS underperform on these benchmarks, thus emphasizing the importance of optimally choosing the space for constructing inliers and outliers.
% It must be noted that the validation split of each of the ID MedMNIST dataset ($i$) after the removal of classes unseen during training, is used as the inlier distribution to the detector. Considering validation samples from each of the other datasets ($j \neq i$) as the respective outlier distributions, we compute the average and std. deviation of AUROC. We also similarly report the AUPR metrics in the appendix.   

\paragraph{Near OOD Detection on MedMNIST.}In this experiment, we evaluate our approach on open-set recognition (subset of classes held out during training). The inherently homogeneous nature of medical images and subtle variations in the image statistics across classes~\cite{mood} makes this task challenging.  In Table \ref{tab:s_medmnist}, we report the AUROCs for the Near OOD detection task with the $40-2$ WideResNet backbone. Energy-based detectors designed with our approach produce the best performance across all datasets (except for the case of PathMNIST). While the G-ODIN detector (with learned additive noise magnitude) performs competitively in some cases, it incurs a large variance across benchmarks.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.\linewidth]{figs/results.png}
    \caption{\textbf{results}. }
    \label{fig:results}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figs/hist_blood.pdf}
%     \caption{\textbf{Histograms of negative energy scores}. We plot the scores obtained using different inlier and outlier specifications. With Blood MNIST as ID, the top row corresponds to modality shift (OOD: Derma MNIST) and the bottom row shows semantic shift (OOD: Novel classes).}
%     \label{fig:my_label}
% \end{figure}


%%% ISIC Evaluation
% \begin{table}[t]
% \centering
% \caption{\textbf{Evaluation on the ISIC2019 benchmark.} We report AUROC scores obtained with a ResNet-50 model trained on the ISIC2019 dataset. Note, we show results for both Near OOD (blue) and Far OOD (red) settings.}
% \renewcommand{\arraystretch}{1.0}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{|c|cccccc|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \cellcolor[HTML]{EFEFEF}                                   & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Methods}}                                                                                                                                                                                                                            \\ \cline{2-7} 
% \rowcolor[HTML]{EFEFEF} 
% \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{OOD Data}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G-ODIN}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{VOS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{VOS++}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{NDA}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{NDA++}} & \textbf{Ours} \\ \hline
% \hline

% \cellcolor[HTML]{e6f3ff} Novel Classes &  \multicolumn{1}{c|}{62.20} & \multicolumn{1}{c|}{\cellcolor[HTML]{C6F7C6}75.04} & \multicolumn{1}{c|}{68.69} & \multicolumn{1}{c|}{65.41} & \multicolumn{1}{c|}{68.38} & \cellcolor[HTML]{FFDBB0}74.00 \\ \hline \hline 

% \cellcolor[HTML]{e6f3ff} Clin Skin & \multicolumn{1}{c|}{62.93} & \multicolumn{1}{c|}{61.33} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}78.80} & \multicolumn{1}{c|}{67.06} & \multicolumn{1}{c|}{72.01} & \cellcolor[HTML]{C6F7C6}81.55 \\ \hline \hline 

% \cellcolor[HTML]{e6f3ff} Derm Skin  & \multicolumn{1}{c|}{71.93} & \multicolumn{1}{c|}{80.53} & \multicolumn{1}{c|}{79.27} & \multicolumn{1}{c|}{82.73} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}85.5} & \cellcolor[HTML]{C6F7C6}93.9 \\ \hline \hline 

% \cellcolor[HTML]{ffebe6} Wilds  & \multicolumn{1}{c|}{65.78} & \multicolumn{1}{c|}{66.71} & \multicolumn{1}{c|}{57.15} & \multicolumn{1}{c|}{83.69} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}85.29} & \cellcolor[HTML]{C6F7C6}99.77 \\ \hline \hline 

% \cellcolor[HTML]{ffebe6} Colorectal  & \multicolumn{1}{c|}{77.08} & \multicolumn{1}{c|}{32.02} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}81.27} & \multicolumn{1}{c|}{71.33} & \multicolumn{1}{c|}{78.84} & \cellcolor[HTML]{C6F7C6}98.58 \\ \hline \hline 

% \cellcolor[HTML]{ffebe6} Knee & \multicolumn{1}{c|}{66.50} & \multicolumn{1}{c|}{23.02} & \multicolumn{1}{c|}{83.47} & \multicolumn{1}{c|}{89.25} & \multicolumn{1}{c|}{\cellcolor[HTML]{C6F7C6}94.73} & \cellcolor[HTML]{FFDBB0}94.08 \\ \hline \hline 

% \cellcolor[HTML]{ffebe6} CXR  & \multicolumn{1}{c|}{74.32} & \multicolumn{1}{c|}{76.80} & \multicolumn{1}{c|}{80.93} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}83.18} & \multicolumn{1}{c|}{62.08} & \cellcolor[HTML]{C6F7C6}96.94 \\ \hline \hline 

% \cellcolor[HTML]{ffebe6} Retina & \multicolumn{1}{c|}{71.10} & \multicolumn{1}{c|}{76.33} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFDBB0}87.39} & \multicolumn{1}{c|}{76.04} & \multicolumn{1}{c|}{76.65} & \cellcolor[HTML]{C6F7C6}95.86 \\
% \hline\hline
% Avg. & \multicolumn{1}{c|}{68.98} & \multicolumn{1}{c|}{61.47} & \multicolumn{1}{c|}{77.12} & \multicolumn{1}{c|}{77.34} & \multicolumn{1}{c|}{77.94} & \textbf{91.84} \\
%  \hline
% \end{tabular}
% }
% \vspace{-0.2in}

% \label{tab:s+d_isic}
% \end{table}

\paragraph{Detection Results on ISIC2019.} Next, we perform evaluations on the ISIC2019 Skin Lesion benchmark, which contains higher resolution images ($224 \times 224$) and represents different types of lesions. Note, we vary the architecture of the backbone (Resnet-50~\cite{He_2016_CVPR}) to understand the generality of our method. Similar to the previous experiment, we consider a suite of Near and Far OOD data, and evaluate performance using AUROC (additional evaluations are included in the appendix). Table \ref{tab:s+d_isic} provides the results across the different OOD settings. In each case, the OOD scenarios are appropriately categorized into Near (blue) and Far (red) OOD respectively. We observe that our approach improves upon other state-of-the-art approaches by significant margins. For example, our method achieves average improvements of $22\%$ and $30\%$ over G-ODIN and the VOS baselines. 

% It can be observed that on this benchmark, NDA achieves detection accuracies that are comparable to our approach, particular in the case of modality shifts.  and Colorectal cancer histopathology benchmark   %s \ref{tab:s+d_colorectal} It can be observed that, in the case of ISIC2019, our approach improves upon state-of-the-art methods, namely G-ODIN and VOS, by margins of $22\%$ and $13\%$ respectively.

\section{Discussion} From the empirical results in this study,  we conclude that the space in which the inlier/oitlier augmentations are specified plays a crucial role in producing improved OOD detectors. Importantly, the inherent diversity offered by the pixel-space outlier synthesis is essential for accurate far OOD detection. This behavior is further emphasized by the observation that NDA \& NDA++ produce improved detection scores over VOS and VOS++ baslines, which synthesize latent-space outliers with limited diversity. On the other hand, for open-set recognition, we find that VOS and VOS++ typically work better than NDA and G-ODIN. Interestingly, our approach which samples hard inliers in the latent space is particularly effective at further improving the detector sensitivity for Near-OOD. Overall, by calibrating the OOD detector using our proposed approach, we obtain improved OOD detection on all medical imaging benchmarks. Figure \ref{fig:my_label} depicts the histograms of the negative energy scores for the case of BloodMNIST (ID), wherein the modality shift results were obtained using DermaMNIST and the semantic shift corresponds to novel classes. We observe that our approach effectively distinguishes between ID and OOD distributions (much higher scores for ID data) in both cases, as illustrated by well-separated distributions, while the other approaches contain high overlap in their scores.


%  We also make the surprising finding that vanilla ODIN is a very strong baseline for medical OOD problems and tends to outperform its sophisticated variant G-ODIN.
% We also identify that our proposed approach produces significantly higher energy scores for ID data in comparison to OOD producing well-separated distributions (Histograms of energy scores are provided in the appendix), while other approaches contain high overlap in their scores.
          



